Mapping the Morphology and Kinematics of a Lyman-alpha-selected Nebula at z=3.15 with MUSE

Recent wide-field integral field spectroscopy has revealed the detailed properties of high redshift Lyman-alpha (Lya) nebulae, most often targeted due to the presence of an active galactic nucleus (AGN). Here, we use VLT/MUSE to resolve the morphology and kinematics of a nebula initially identified due to strong Lya emission at $z\sim3.2$ (LABn06; Nilsson et al. 2006). Our observations reveal a two-lobed Lya nebula, at least $\sim$173 pkpc in diameter, with a light-weighted centroid near a mid-infrared source (within $\approx$17.2 pkpc) that appears to host an obscured AGN. The Lya emission near the AGN is also coincident in velocity with the kinematic center of the nebula, suggesting that the nebula is both morphologically and kinematically centered on the AGN. Compared to AGN-selected Lya nebulae, the surface brightness profile of this nebula follows a typical exponential profile at large radii ($>$25 pkpc), although at small radii, the profile shows an unusual dip at the location of the AGN. The kinematics and asymmetry are similar to, and the CIV and HeII upper limits are consistent with other AGN-powered Lya nebulae. Double-peaked and asymmetric line profiles suggest that Lya resonant scattering may be important in this nebula. These results support the picture of the AGN being responsible for powering a Lya nebula that is oriented roughly in the plane of the sky. Further observations will explore whether the central surface brightness depression is indicative of either an unusual gas or dust distribution or variation in the ionizing output of the AGN over time.

==> Sanderson_2021(arXiv_version)/Flux_Measurements_table.tex <==
Full & 175.35 & $<$28.57 & $<$16.18 & $<$26.61 & $<$11.24 \\
A & 10.73 & $<$2.85 & $<$1.25 & $<$1.89 & $<$1.89 \\
B & 8.59 & $<$2.63 & $<$1.81 & $<$1.63 & $<$1.54 \\
C & 7.48 & $<$1.56 & $<$1.41 & $<$2.3 & $<$2.48 \\
D & 8.07 & $<$2.15 & $<$1.72 & $<$2.46 & $<$4.78 \\
S6 & 3.23 & $<$0.28 & $<$0.43 & $<$0.46 & $<$0.66 \\
